Aligning GPTRec with Beyond-Accuracy Goals with Reinforcement Learning

Adaptations of Transformer models, such as BERT4Rec and SASRec, achieve state-of-the-art performance in the sequential recommendation task according to accuracy-based metrics, such as NDCG. These models treat items as tokens and then utilise a score-and-rank approach (Top-K strategy), where the model first computes item scores and then ranks them according to this score. While this approach works well for accuracy-based metrics, it is hard to use it for optimising more complex beyond-accuracy metrics such as diversity. Recently, the GPTRec model, which uses a different Next-K strategy, has been proposed as an alternative to the Top-K models. In contrast with traditional Top-K recommendations, Next-K generates recommendations item-by-item and, therefore, can account for complex item-to-item interdependencies important for the beyond-accuracy measures. However, the original GPTRec paper focused only on accuracy in experiments and needed to address how to optimise the model for complex beyond-accuracy metrics. Indeed, training GPTRec for beyond-accuracy goals is challenging because the interaction training data available for training recommender systems typically needs to be aligned with beyond-accuracy recommendation goals. To solve the misalignment problem, we train GPTRec using a 2-stage approach: in the first stage, we use a teacher-student approach to train GPTRec, mimicking the behaviour of traditional Top-K models; in the second stage, we use Reinforcement Learning to align the model for beyond-accuracy goals. In particular, we experiment with increasing recommendation diversity and reducing popularity bias. Our experiments on two datasets show that in 3 out of 4 cases, GPTRec's Next-K generation approach offers a better tradeoff between accuracy and secondary metrics than classic greedy re-ranking techniques.

==> tables/embeddings_reduction.tex <==
\begin{tabular}{lll|ccc|ccc|ccc}
\toprule
Dataset & Num Items & \makecell[l]{GPU Memory \\ (one-token-per-item \\ mode)} & 
\makecell{t=2 \\ v=128 \\ (256 embs;\\ 0.25 MB)} & 
\makecell{t=2 \\ v=512 \\ (1024 embs;\\ 1.00 MB)} & 
\makecell{t=2 \\ v=2048 \\ (4096 embs;\\ 4.00 MB)} & 
\makecell{t=4 \\ v=128 \\ (512 embs;\\ 0.50 MB)} & 
\makecell{t=4 \\ v=512 \\ (2048 embs;\\ 2.00 MB)} & 
\makecell{t=4 \\ v=2048 \\ (8192 embs;\\ 8.00 MB)} & 
\makecell{t=8 \\ v=128 \\ (1024 embs;\\ 1.00 MB)} & 
\makecell{t=8 \\ v=512 \\ (4096 embs;\\ 4.00 MB)} & 
\makecell{t=8 \\ v=2048 \\ (16384 embs;\\ 16.00 MB)} \\
\midrule
MovieLens-1M & 3,416 & 3.34 MB & 7.494\% & 29.977\% & 119.906\% & 14.988\% & 59.953\% & 239.813\% & 29.977\% & 119.906\% & 479.625\% \\
MovieLens-20M & 138,493 & 135.25 MB & 0.185\% & 0.739\% & 2.958\% & 0.370\% & 1.479\% & 5.915\% & 0.739\% & 2.958\% & 11.830\% \\
Yelp & 150,346 & 146.82 MB & 0.170\% & 0.681\% & 2.724\% & 0.341\% & 1.362\% & 5.449\% & 0.681\% & 2.724\% & 10.898\% \\
Gowalla & 1,280,969 & 1.22 GB & 0.020\% & 0.080\% & 0.320\% & 0.040\% & 0.160\% & 0.640\% & 0.080\% & 0.320\% & 1.279\% \\
Amazon Books & 5,264,307 & 5.02 GB & 0.005\% & 0.019\% & 0.078\% & 0.010\% & 0.039\% & 0.156\% & 0.019\% & 0.078\% & 0.311\% \\
LastFM-1b & 32,291,134 & 30.80 GB & 0.001\% & 0.003\% & 0.013\% & 0.002\% & 0.006\% & 0.025\% & 0.003\% & 0.013\% & 0.051\% \\
\bottomrule
\end{tabular}


==> tables/model_performance.tex <==
\begin{tabular}{lllll|ll}
\toprule
Model name & Generation Strategy & Architecture & Training Task & Loss & Recall@10 & NDCG@10 \\
\midrule
BERT4Rec & TopK & Encoder & MLM (Item Masking) & Cross Entropy (Softmax Loss) & \textbf{0.282} & \textbf{0.152} \\
GPTRec-TopK & TopK & Decoder & LM (Sequence Shifting) & Cross Entropy (Softmax Loss) & \underline{0.254} & \underline{0.146} \\
SASRec & TopK & Decoder & LM (Sequence Shifting) & Binary Cross-Entropy & 0.199 & 0.108 \\
GPTRec-NextK & NextK & Decoder & LM (Sequence Shifting) & Cross Entropy (Softmax Loss) & 0.157 & 0.105 \\
\bottomrule
\end{tabular}

